LCM from FCA Point of View: A CbO-style Algorithm with Speed-up Features

LCM is an algorithm for enumeration of frequent closed itemsets in transaction databases. It is well known that when we ignore the required frequency, the closed itemsets are exactly intents of formal concepts in Formal Concept Analysis (FCA). We describe LCM in terms of FCA and show that LCM is basically the Close-by-One algorithm with multiple speed-up features for processing sparse data. We analyze the speed-up features and compare them with those of similar FCA algorithms, like FCbO and algorithms from the In-Close family.

==> fig1.tex <==
% !TeX encoding = UTF-8
% !TeX spellcheck = en_US
% !TeX root= text.tex

% !TeX encoding = UTF-8
% !TeX spellcheck = en_US
% !TeX root= CbO.tex

\begin{center}
\begin{tikzpicture}[xscale=1.5]
\node (0L) at (1,0) {$\emptyset$};
\node[circle,draw] (0) at (1,0) {~~~};

\node (2L) at (-2,-1) {1};
\node[circle,draw] (2) at (2L) {~~~};

\node (3L) at (0,-1) {2};
\node[circle,draw] (3) at (3L) {~~~};

\node (4L) at (2,-1) {3};
\node[circle,draw] (4) at (4L) {~~~};

\node (5L) at (4,-1) {4};
\node[circle,draw] (5) at (5L) {~~~};

\node (45L) at (2,-2) {4};
\node[circle,draw] (45) at (45L) {~~~};

\node (34L) at (-.5,-2) {3};
\node[circle,draw] (34) at (34L) {~~~};

\node (35L) at (.5,-2) {4};
\node[circle,draw] (35) at (35L) {~~~};

\node (345L) at (-.5,-3) {4};
\node[circle,draw] (345) at (345L) {~~~};



\begin{scope}[xshift=-3cm,yshift=-1cm]

\node (23L) at (0,-1) {2};
\node[circle,draw] (23) at (23L) {~~~};

\node (24L) at (1,-1) {3};
\node[circle,draw] (24) at (24L) {~~~};

\node (25L) at (2,-1) {4};
\node[circle,draw] (25) at (25L) {~~~};

\node (245L) at (1,-2) {4};
\node[circle,draw] (245) at (245L) {~~~};

\node (234L) at (-.5,-2) {3};
\node[circle,draw] (234) at (234L) {~~~};

\node (235L) at (.5,-2) {4};
\node[circle,draw] (235) at (235L) {~~~};

\node (2345L) at (-.5,-3) {4};
\node[circle,draw] (2345) at (2345L) {~~~};
\end{scope}

\draw (0) -- (2);
\draw (0) -- (3);
\draw (0) -- (4);
\draw (0) -- (5);

\draw (2) -- (23);
\draw (2) -- (24);
\draw (2) -- (25);

\draw (3) -- (34);
\draw (3) -- (35);

\draw (4) -- (45);

\draw (23) -- (234);
\draw (23) -- (235);

\draw (24) -- (245);
\draw (34) -- (345);

\draw (234) -- (2345);



\node[fill=white,inner sep=1.5pt] (0L) at (0.north west) {\tiny 1};
\node[fill=white,inner sep=1.5pt] (2L) at (2.north west) {\tiny 2};
\node[fill=white,inner sep=1.5pt] (3L) at (3.north west) {\tiny 10};
\node[fill=white,inner sep=1.5pt] (4L) at (4.north west) {\tiny 14};
\node[fill=white,inner sep=1.5pt] (5L) at (5.north west) {\tiny 16};
\node[fill=white,inner sep=1.5pt] (45L) at (45.north west) {\tiny 15};
\node[fill=white,inner sep=1.5pt] (34L) at (34.north west) {\tiny 11};
\node[fill=white,inner sep=1.5pt] (35L) at (35.north west) {\tiny 13};
\node[fill=white,inner sep=1.5pt] (345L) at (345.north west) {\tiny 12};
\node[fill=white,inner sep=1.5pt] (23L) at (23.north west) {\tiny 3};
\node[fill=white,inner sep=1.5pt] (24L) at (24.north west) {\tiny 7};
\node[fill=white,inner sep=1.5pt] (25L) at (25.north west) {\tiny 9};
\node[fill=white,inner sep=1.5pt] (245L) at (245.north west) {\tiny 8};
\node[fill=white,inner sep=1.5pt] (234L) at (234.north west) {\tiny 4};
\node[fill=white,inner sep=1.5pt] (235L) at (235.north west) {\tiny 6};
\node[fill=white,inner sep=1.5pt] (2345L) at (2345.north west) {\tiny 5};


\draw[dotted,-latex] (0L) -- (2L);
\draw[dotted,-latex] (2L) -- (23L);
\draw[dotted,-latex] (23L) -- (234L);
\draw[dotted,-latex] (234L) -- (2345L);
\draw[dotted,-latex] (2345L) -- (235L);
\draw[dotted,-latex] (235L) -- (24L);
\draw[dotted,-latex] (24L) -- (245L);
\draw[dotted,-latex] (245L) -- (25L);
\draw[dotted,-latex] (25L) -- (3L);
\draw[dotted,-latex] (3L) -- (34L);
\draw[dotted,-latex] (34L) -- (345L);
\draw[dotted,-latex] (345L) -- (35L);
\draw[dotted,-latex] (35L) -- (4L);
\draw[dotted,-latex] (4L) -- (45L);
\draw[dotted,-latex] (45L) -- (5L);

%%%% path

%\draw[dashed] plot[smooth,tension = 1] coordinates { (0.north west) (2.north west) (23.north west) (234.north west) (2345.west)
% (2345.south east) (235.south) (235.east) (24.west)
%};


\end{tikzpicture}
\end{center}

%
%\begin{center}
%\begin{tikzpicture}[xscale=1.5]
%\node[draw,circle] (0) at (1,0) {$\emptyset$};
%
%\node[draw,circle] (2) at (-2,-1) {1};
%\node[draw,circle] (3) at (0,-1) {2};
%\node (4) at (2,-1) {3};
%\node (5) at (4,-1) {4};
%\node (45) at (2,-2) {4};
%\node (34) at (-.5,-2) {3};
%
%
%
%
%\node (35) at (.5,-2) {4};
%
%\node (345) at (-.5,-3) {4};
%
%\begin{scope}[xshift=-3cm,yshift=-1cm]
%
%\node (23) at (0,-1) {2};
%
%\node (24) at (1,-1) {3};
%\node (25) at (2,-1) {4};
%\node[draw,circle] (245) at (1,-2) {4};
%
%
%\node[draw,circle] (234) at (-.5,-2) {3};
%\node (235) at (.5,-2) {4};
%
%\node[draw,circle] (2345) at (-.5,-3) {4};
%\end{scope}
%
%\draw (0) -- (2);
%\draw (0) -- (3);
%\draw (0) -- (4);
%\draw (0) -- (5);
%
%\draw (2) -- (23);
%\draw (2) -- (24);
%\draw (2) -- (25);
%
%\draw (3) -- (34);
%\draw (3) -- (35);
%
%\draw (4) -- (45);
%
%\draw (23) -- (234);
%\draw (23) -- (235);
%
%\draw (24) -- (245);
%\draw (34) -- (345);
%
%\draw (234) -- (2345);
%
%\path[->,dotted] (34) edge[bend left=30] (2345);
%
%\end{tikzpicture}
%\end{center}
  

==> fig3.tex <==
% !TeX encoding = UTF-8
% !TeX spellcheck = en_US
% !TeX root= text.tex

\begin{center}
\begin{tikzpicture}[xscale=1.5,yscale=1.4]

\node (0L) at (1,0) {$\emptyset$};
\node[draw,circle] (0) at (0L) {~~~};

\node (2L) at (-2,-1) {$1$};
\node[draw,circle] (2) at (2L) {~~~};

\node (3L) at (0,-1) {$2$};
\node[draw,circle] (3) at (3L) {~~~};

\node (4L) at (2,-1) {$3$};
\node[draw,circle] (4) at (4L) {~~~};

\node (5L) at (4,-1) {$4$};
\node[draw,circle] (5) at (5L) {~~~};



\node (45) at (2.5,-2) {$4$};
\node[draw,circle] (34) at (-.5,-2) {$3$};
\node (35) at (0,-2) {$4$};
%
\node (345) at (-.5,-3) {$4$};


\node[anchor=west, text width=4.8cm] (4F) at (2.5, -3) {\small 1) canonicity test fails;\\ store: %(\emptyset \cup \{4\})^{\up\down}$ 
 4~adds~1 };

\path[-latex,draw,dotted] (4F) -- (5);


\node[anchor=west, text width=5cm] (4FF) at (0.5, -4.5) {\small 2) stored information \\ reused for $\{2\}, \{3\}, \{2,3\}$};


\path[-latex,draw,dotted] (4FF) -- (3);
\path[-latex,draw,dotted] (4FF) -- (4);
\path[-latex,draw,dotted] (4FF) -- (34);

%
%\begin{scope}[xshift=-3cm,yshift=-1cm]
%
%\node (23) at (0,-1) {2};
%
%\node (24) at (1,-1) {3};
%\node (25) at (2,-1) {4};
%\node (245) at (1,-2) {4};
%
%
%\node (234) at (-.5,-2) {3};
%\node (235) at (.5,-2) {4};
%
%\node (2345) at (-.5,-3) {4};
%\end{scope}

\draw (0) -- (2);
\draw (0) -- (3);
\draw (0) -- (4);
\draw (0) -- (5);

\draw[dashed] (2) -- (-3,-3) -- (-1,-3) -- (2);
%\draw (2) -- (24);
%\draw (2) -- (25);
%
\draw (3) -- (34);
\draw (3) edge node {\LARGE\x}  (35);

%
\draw (4) edge node {\LARGE\x} (45);
%
%\draw (23) -- (234);
%\draw (23) -- (235);
%
%\draw (24) -- (245);
\draw (34) edge node {\LARGE\x} (345);
%
%\draw (234) -- (2345);

\end{tikzpicture}
\end{center}


==> fig_occurence_deliver.tex <==
\begin{figure}
\begin{tikzpicture}
\begin{scope}
\node at (0,0) {%
\begin{tabular}{c|l}
        & items \\\hline
  a     & 2 3 4 5 7 8 \\
  b     & 1 2 3 4 5 7 \\
  c     & 2 3 6 7 \\
  d,i   & 2 7 8 \\
  e,f,h & 1 3 5 6 7 \\
  g     & 5 7
\end{tabular}};

%\draw[dotted,very thick,-latex] (-1.4,.8) -- (1.8,.8);

\node[rectangle] at (3,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
1
\end{tabular}
};
 
\node[rectangle] at (4,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
2
\end{tabular}
};

\node[rectangle] at (5,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
3
\end{tabular}
};
 
\node[rectangle] at (6,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
4
\end{tabular}
};

\node[rectangle] at (7,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
5
\end{tabular}
};

\node[rectangle] at (8,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
6
\end{tabular}
};
 
\node[rectangle] at (9,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
7
\end{tabular}
};

\node[rectangle] at (10,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
8
\end{tabular}
};
\end{scope}


\begin{scope}[yshift=-4cm]
\node at (0,0) {%
\begin{tabular}{c|l}
        & items \\\hline
  a     & 2 3 4 5 7 8 \\
  b     & 1 2 3 4 5 7 \\
  c     & 2 3 6 7 \\
  d,i   & 2 7 8 \\
  e,f,h & 1 3 5 6 7 \\
  g     & 5 7
\end{tabular}};

\draw[dotted,very thick,-latex] (-1.4,.8) -- (1.8,.8);

\node[rectangle] at (3,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
1
\end{tabular}
};
 
\node[rectangle] at (4,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
2
\end{tabular}
};

\node[rectangle] at (5,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
3
\end{tabular}
};
 
\node[rectangle] at (6,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
4
\end{tabular}
};

\node[rectangle] at (7,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
5
\end{tabular}
};

\node[rectangle] at (8,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
6
\end{tabular}
};
 
\node[rectangle] at (9,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
7
\end{tabular}
};

\node[rectangle] at (10,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
8
\end{tabular}
};
\end{scope}

\begin{scope}[yshift=-8cm]
\node at (0,0) {%
\begin{tabular}{c|l}
        & items \\\hline
  a     & 2 3 4 5 7 8 \\
  b     & 1 2 3 4 5 7 \\
  c     & 2 3 6 7 \\
  d,i   & 2 7 8 \\
  e,f,h & 1 3 5 6 7 \\
  g     & 5 7
\end{tabular}};

\draw[dotted,very thick,-latex] (-1.4,.4) -- (1.8,.4);

\node[rectangle] at (3,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
b \\\hline
\end{tabular}\\
1
\end{tabular}
};
 
\node[rectangle] at (4,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
b \\
a \\\hline
\end{tabular}\\
2
\end{tabular}
};

\node[rectangle] at (5,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
b \\
a \\\hline
\end{tabular}\\
3
\end{tabular}
};
 
\node[rectangle] at (6,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
b \\
a \\\hline
\end{tabular}\\
4
\end{tabular}
};

\node[rectangle] at (7,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
b \\
a \\\hline
\end{tabular}\\
5
\end{tabular}
};

\node[rectangle] at (8,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
6
\end{tabular}
};
 
\node[rectangle] at (9,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
b \\
a \\\hline
\end{tabular}\\
7
\end{tabular}
};

\node[rectangle] at (10,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
8
\end{tabular}
};
\end{scope}



\begin{scope}[yshift=-12cm]
\node at (0,0) {%
\begin{tabular}{c|l}
        & items \\\hline
  a     & 2 3 4 5 7 8 \\
  b     & 1 2 3 4 5 7 \\
  c     & 2 3 6 7 \\
  d,i   & 2 7 8 \\
  e,f,h & 1 3 5 6 7 \\
  g     & 5 7
\end{tabular}};

\draw[dotted,very thick,-latex] (-1.4,0) -- (1.8,0);
\draw[dotted,very thick,-latex] (-1.4,-.39) -- (1.8,-.39);
\draw[dotted,very thick,-latex] (-1.4,-.78) -- (1.8,-.78);
\draw[dotted,very thick,-latex] (-1.4,-1.17) -- (1.8,-1.17);

\node[rectangle] at (3,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
e,f,h \\
b \\\hline
\end{tabular}\\
1
\end{tabular}
};
 
\node[rectangle] at (4,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
d,i \\
c \\
b \\
a \\\hline
\end{tabular}\\
2
\end{tabular}
};

\node[rectangle] at (5,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
e,f,h \\
c \\
b \\
a \\\hline
\end{tabular}\\
3
\end{tabular}
};
 
\node[rectangle] at (6,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
b \\
a \\\hline
\end{tabular}\\
4
\end{tabular}
};

\node[rectangle] at (7,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
g \\
e,f,h \\
b \\
a \\\hline
\end{tabular}\\
5
\end{tabular}
};

\node[rectangle] at (8,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
e,f,h \\
c \\\hline
\end{tabular}\\
6
\end{tabular}
};
 
\node[rectangle] at (9,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
g \\
e,f,h \\
d,i \\
c \\
b \\
a \\\hline
\end{tabular}\\
7
\end{tabular}
};

\node[rectangle] at (10,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
d,i \\
a \\\hline
\end{tabular}\\
8
\end{tabular}
};
\end{scope}
\end{tikzpicture}
\caption{Occurrence deliver in LCM. \label{fig:occdel}}
\end{figure}


%\begin{figure}
%\begin{center}
%\scalebox{.9}{%
%\begin{tikzpicture}
%
%\begin{scope}
%\node (a) {%
%\begin{tabular}{ll|cccccccc}
%&     & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\\hline
%$\Rightarrow$&{a}~~&   &\x &\x &\x &\x &   &\x &\x \\
%&{b}  &\x &\x &\x &\x &\x &   &\x &   \\
%&{c}  &   &\x &\x &   &   &\x &\x &   \\
%&{d}  &   &\x &   &   &   &   &\x &\x \\
%&{e}  &\x &   &\x &   &\x &\x &\x &   \\
%&{f}  &\x &   &\x &   &\x &\x &\x &   \\
%&{g}  &   &   &   &   &\x &   &\x &   \\
%&{h}  &   &   &\x &   &\x &\x &\x &   \\
%&{i}  &   &\x &   &   &   &   &   &\x \\
%\end{tabular}
%};
%
%
%
%\node[anchor=west] (a) at (6,0) {%
%\begin{tabular}{l|l}
%bucket\,{1}~~&  \\
%bucket\,{2}  & a \\
%bucket\,{3}  & a \\
%bucket\,{4}  & a \\
%bucket\,{5}  & a \\
%bucket\,{6}  &  \\
%bucket\,{7}  & a \\
%bucket\,{8}  & a \\
%\end{tabular}
%};
%\end{scope}
%
%\begin{scope}[yshift=-4.5cm]
%\node (a) {%
%\begin{tabular}{ll|cccccccc}
%&     & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\\hline
%&{a}~~&   &\x &\x &\x &\x &   &\x &\x \\
%$\Rightarrow$&{b}  &\x &\x &\x &\x &\x &   &\x &   \\
%&{c}  &   &\x &\x &   &   &\x &\x &   \\
%&{d}  &   &\x &   &   &   &   &\x &\x \\
%&{e}  &\x &   &\x &   &\x &\x &\x &   \\
%&{f}  &\x &   &\x &   &\x &\x &\x &   \\
%&{g}  &   &   &   &   &\x &   &\x &   \\
%&{h}  &   &   &\x &   &\x &\x &\x &   \\
%&{i}  &   &\x &   &   &   &   &   &\x \\
%\end{tabular}
%};
%
%
%
%\node[anchor=west] (a) at (6,0) {%
%\begin{tabular}{l|l}
%bucket\,{1}~~& b \\
%bucket\,{2}  & a,b \\
%bucket\,{3}  & a,b \\
%bucket\,{4}  & a,b \\
%bucket\,{5}  & a,b \\
%bucket\,{6}  &  \\
%bucket\,{7}  & a,b \\
%bucket\,{8}  & a \\
%\end{tabular}
%};
%\end{scope}
%
%\begin{scope}[yshift=-9cm]
%\node (a) {%
%\begin{tabular}{ll|cccccccc}
%&     & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\\hline
%&{a}~~&   &\x &\x &\x &\x &   &\x &\x \\
%&{b}  &\x &\x &\x &\x &\x &   &\x &   \\
%$\Rightarrow$&{c}  &   &\x &\x &   &   &\x &\x &   \\
%&{d}  &   &\x &   &   &   &   &\x &\x \\
%&{e}  &\x &   &\x &   &\x &\x &\x &   \\
%&{f}  &\x &   &\x &   &\x &\x &\x &   \\
%&{g}  &   &   &   &   &\x &   &\x &   \\
%&{h}  &   &   &\x &   &\x &\x &\x &   \\
%&{i}  &   &\x &   &   &   &   &   &\x \\
%\end{tabular}
%};
%
%
%
%\node[anchor=west] (a) at (6,0) {%
%\begin{tabular}{l|l}
%bucket\,{1}~~& b \\
%bucket\,{2}  & a,b,c \\
%bucket\,{3}  & a,b,c \\
%bucket\,{4}  & a,b \\
%bucket\,{5}  & a,b \\
%bucket\,{6}  & c, \\
%bucket\,{7}  & a,b,c \\
%bucket\,{8}  & a \\
%\end{tabular}
%};
%\end{scope}
%
%\end{tikzpicture}}
%\end{center}
%\caption{Occurence deliver (computation of extents), processing first three rows.\label{fig:occdel}}
%\end{figure}


==> fig_occurence_deliver_small.tex <==
\begin{figure}[t]
\scalebox{.47}{
\begin{tikzpicture}
\begin{scope}

\node[anchor=west] at (-1,2) {\LARGE 1) before occurence deliver};

\node at (0,0) {%
\begin{tabular}{c|l}
        & items \\\hline
  a     & 2 3 4 5 7 8 \\
  b     & 1 2 3 4 5 7 \\
  c     & 2 3 6 7 \\
  d,i   & 2 7 8 \\
  e,f,h & 1 3 5 6 7 \\
  g     & 5 7
\end{tabular}};

%\draw[dotted,very thick,-latex] (-1.4,.8) -- (1.8,.8);

\node[rectangle] at (3,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
1
\end{tabular}
};
 
\node[rectangle] at (4,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
2
\end{tabular}
};

\node[rectangle] at (5,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
3
\end{tabular}
};
 
\node[rectangle] at (6,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
4
\end{tabular}
};

\node[rectangle] at (7,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
5
\end{tabular}
};

\node[rectangle] at (8,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
6
\end{tabular}
};
 
\node[rectangle] at (9,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
7
\end{tabular}
};

\node[rectangle] at (10,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
8
\end{tabular}
};
\end{scope}


\begin{scope}[xshift=13.5cm]

\node[anchor=west] at (-1,2) {\LARGE 2) processing first row (object a)};

\node at (0,0) {%
\begin{tabular}{c|l}
        & items \\\hline
  a     & 2 3 4 5 7 8 \\
  b     & 1 2 3 4 5 7 \\
  c     & 2 3 6 7 \\
  d,i   & 2 7 8 \\
  e,f,h & 1 3 5 6 7 \\
  g     & 5 7
\end{tabular}};

\draw[dotted,very thick,-latex] (-1.4,.8) -- (1.8,.8);

\node[rectangle] at (3,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
1
\end{tabular}
};
 
\node[rectangle] at (4,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
2
\end{tabular}
};

\node[rectangle] at (5,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
3
\end{tabular}
};
 
\node[rectangle] at (6,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
4
\end{tabular}
};

\node[rectangle] at (7,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
5
\end{tabular}
};

\node[rectangle] at (8,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
6
\end{tabular}
};
 
\node[rectangle] at (9,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
7
\end{tabular}
};

\node[rectangle] at (10,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
8
\end{tabular}
};
\end{scope}

\begin{scope}[yshift=-5cm]

\node[anchor=west] at (-1,2) {\LARGE 3) processing second row (object b)};

\node at (0,0) {%
\begin{tabular}{c|l}
        & items \\\hline
  a     & 2 3 4 5 7 8 \\
  b     & 1 2 3 4 5 7 \\
  c     & 2 3 6 7 \\
  d,i   & 2 7 8 \\
  e,f,h & 1 3 5 6 7 \\
  g     & 5 7
\end{tabular}};

\draw[dotted,very thick,-latex] (-1.4,.4) -- (1.8,.4);

\node[rectangle] at (3,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
b \\\hline
\end{tabular}\\
1
\end{tabular}
};
 
\node[rectangle] at (4,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
b \\
a \\\hline
\end{tabular}\\
2
\end{tabular}
};

\node[rectangle] at (5,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
b \\
a \\\hline
\end{tabular}\\
3
\end{tabular}
};
 
\node[rectangle] at (6,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
b \\
a \\\hline
\end{tabular}\\
4
\end{tabular}
};

\node[rectangle] at (7,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
b \\
a \\\hline
\end{tabular}\\
5
\end{tabular}
};

\node[rectangle] at (8,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
~ \\\hline
\end{tabular}\\
6
\end{tabular}
};
 
\node[rectangle] at (9,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
b \\
a \\\hline
\end{tabular}\\
7
\end{tabular}
};

\node[rectangle] at (10,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
~ \\
a \\\hline
\end{tabular}\\
8
\end{tabular}
};
\end{scope}



\begin{scope}[xshift=13.5cm,yshift=-5cm]

\node[anchor=west] at (-1,2) {\LARGE 4) processing the rest (objects c--g)};

\node at (0,0) {%
\begin{tabular}{c|l}
        & items \\\hline
  a     & 2 3 4 5 7 8 \\
  b     & 1 2 3 4 5 7 \\
  c     & 2 3 6 7 \\
  d,i   & 2 7 8 \\
  e,f,h & 1 3 5 6 7 \\
  g     & 5 7
\end{tabular}};

\draw[dotted,very thick,-latex] (-1.4,0) -- (1.8,0);
\draw[dotted,very thick,-latex] (-1.4,-.39) -- (1.8,-.39);
\draw[dotted,very thick,-latex] (-1.4,-.78) -- (1.8,-.78);
\draw[dotted,very thick,-latex] (-1.4,-1.17) -- (1.8,-1.17);

\node[rectangle] at (3,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
e,f,h \\
b \\\hline
\end{tabular}\\
1
\end{tabular}
};
 
\node[rectangle] at (4,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
d,i \\
c \\
b \\
a \\\hline
\end{tabular}\\
2
\end{tabular}
};

\node[rectangle] at (5,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
e,f,h \\
c \\
b \\
a \\\hline
\end{tabular}\\
3
\end{tabular}
};
 
\node[rectangle] at (6,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
b \\
a \\\hline
\end{tabular}\\
4
\end{tabular}
};

\node[rectangle] at (7,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
g \\
e,f,h \\
b \\
a \\\hline
\end{tabular}\\
5
\end{tabular}
};

\node[rectangle] at (8,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
e,f,h \\
c \\\hline
\end{tabular}\\
6
\end{tabular}
};
 
\node[rectangle] at (9,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
g \\
e,f,h \\
d,i \\
c \\
b \\
a \\\hline
\end{tabular}\\
7
\end{tabular}
};

\node[rectangle] at (10,0) {%
\begin{tabular}{c}
\begin{tabular}{|C{.8cm}|}\hline
~ \\
~ \\
~ \\
~ \\
d,i \\
a \\\hline
\end{tabular}\\
8
\end{tabular}
};
\end{scope}
\end{tikzpicture}}
\caption{Occurrence deliver in LCM. \label{fig:occdel}}
\end{figure}


%\begin{figure}
%\begin{center}
%\scalebox{.9}{%
%\begin{tikzpicture}
%
%\begin{scope}
%\node (a) {%
%\begin{tabular}{ll|cccccccc}
%&     & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\\hline
%$\Rightarrow$&{a}~~&   &\x &\x &\x &\x &   &\x &\x \\
%&{b}  &\x &\x &\x &\x &\x &   &\x &   \\
%&{c}  &   &\x &\x &   &   &\x &\x &   \\
%&{d}  &   &\x &   &   &   &   &\x &\x \\
%&{e}  &\x &   &\x &   &\x &\x &\x &   \\
%&{f}  &\x &   &\x &   &\x &\x &\x &   \\
%&{g}  &   &   &   &   &\x &   &\x &   \\
%&{h}  &   &   &\x &   &\x &\x &\x &   \\
%&{i}  &   &\x &   &   &   &   &   &\x \\
%\end{tabular}
%};
%
%
%
%\node[anchor=west] (a) at (6,0) {%
%\begin{tabular}{l|l}
%bucket\,{1}~~&  \\
%bucket\,{2}  & a \\
%bucket\,{3}  & a \\
%bucket\,{4}  & a \\
%bucket\,{5}  & a \\
%bucket\,{6}  &  \\
%bucket\,{7}  & a \\
%bucket\,{8}  & a \\
%\end{tabular}
%};
%\end{scope}
%
%\begin{scope}[yshift=-4.5cm]
%\node (a) {%
%\begin{tabular}{ll|cccccccc}
%&     & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\\hline
%&{a}~~&   &\x &\x &\x &\x &   &\x &\x \\
%$\Rightarrow$&{b}  &\x &\x &\x &\x &\x &   &\x &   \\
%&{c}  &   &\x &\x &   &   &\x &\x &   \\
%&{d}  &   &\x &   &   &   &   &\x &\x \\
%&{e}  &\x &   &\x &   &\x &\x &\x &   \\
%&{f}  &\x &   &\x &   &\x &\x &\x &   \\
%&{g}  &   &   &   &   &\x &   &\x &   \\
%&{h}  &   &   &\x &   &\x &\x &\x &   \\
%&{i}  &   &\x &   &   &   &   &   &\x \\
%\end{tabular}
%};
%
%
%
%\node[anchor=west] (a) at (6,0) {%
%\begin{tabular}{l|l}
%bucket\,{1}~~& b \\
%bucket\,{2}  & a,b \\
%bucket\,{3}  & a,b \\
%bucket\,{4}  & a,b \\
%bucket\,{5}  & a,b \\
%bucket\,{6}  &  \\
%bucket\,{7}  & a,b \\
%bucket\,{8}  & a \\
%\end{tabular}
%};
%\end{scope}
%
%\begin{scope}[yshift=-9cm]
%\node (a) {%
%\begin{tabular}{ll|cccccccc}
%&     & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\\hline
%&{a}~~&   &\x &\x &\x &\x &   &\x &\x \\
%&{b}  &\x &\x &\x &\x &\x &   &\x &   \\
%$\Rightarrow$&{c}  &   &\x &\x &   &   &\x &\x &   \\
%&{d}  &   &\x &   &   &   &   &\x &\x \\
%&{e}  &\x &   &\x &   &\x &\x &\x &   \\
%&{f}  &\x &   &\x &   &\x &\x &\x &   \\
%&{g}  &   &   &   &   &\x &   &\x &   \\
%&{h}  &   &   &\x &   &\x &\x &\x &   \\
%&{i}  &   &\x &   &   &   &   &   &\x \\
%\end{tabular}
%};
%
%
%
%\node[anchor=west] (a) at (6,0) {%
%\begin{tabular}{l|l}
%bucket\,{1}~~& b \\
%bucket\,{2}  & a,b,c \\
%bucket\,{3}  & a,b,c \\
%bucket\,{4}  & a,b \\
%bucket\,{5}  & a,b \\
%bucket\,{6}  & c, \\
%bucket\,{7}  & a,b,c \\
%bucket\,{8}  & a \\
%\end{tabular}
%};
%\end{scope}
%
%\end{tikzpicture}}
%\end{center}
%\caption{Occurence deliver (computation of extents), processing first three rows.\label{fig:occdel}}
%\end{figure}


==> fig_reduction.tex <==
% !TeX root = text.tex
\begin{figure}
\begin{center}
\scalebox{.9}{%
\begin{tikzpicture}

\node (a) {%
\begin{tabular}{l|cccccccc}
     & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\\hline
{a}~~&   &\x &\x &\x &\x &   &\x &   \\
{b}  &\x &\x &\x &\x &\x &   &\x &   \\
{c}  &   &\x &\x &   &   &\x &\x &   \\
{d}  &   &\x &   &   &   &   &\x &\x \\
{e}  &\x &   &\x &   &\x &\x &\x &   \\
{f}  &\x &\x &\x &   &\x &\x &\x &   \\
{g}  &   &   &   &   &\x &   &\x &   \\
{h}  &   &   &\x &   &\x &\x &\x &   \\
{i}  &   &\x &   &   &   &   &   &\x \\
\end{tabular}
};



\node (b) at (0,-5) {%
\begin{tabular}{l|cccccccc}
     & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\\hline
{a}~~&   &\x &\x &\x &\x &   &\x &   \\
{b}  &\x &\x &\x &\x &\x &   &\x &   \\
{c}  &   &\x &\x &   &   &\x &\x &   \\
%{d}  &   &\x &   &   &   &   &\x &\x \\
{e}  &\x &   &\x &   &\x &\x &\x &   \\
{f}  &\x &   &\x &   &\x &\x &\x &   \\
%{g}  &   &   &   &   &\x &   &\x &   \\
{h}  &   &   &\x &   &\x &\x &\x &   \\
%{i}  &   &\x &   &   &   &   &\x &\x \\
\end{tabular}
};


\node (c) at (0,-9.5) {%
\begin{tabular}{l|cccccc}
     & 1 & 2  & 4 & 5 & 6  \\\hline
{a}~~&   &\x  &\x &\x &       \\
{b}  &\x &\x  &\x &\x &       \\
{c}  &   &\x  &   &   &\x     \\
%{d}  &   &\x &   &   &   &   &\x &\x \\
{e}  &\x &    &   &\x &\x      \\
{f}  &\x &    &   &\x &\x    \\
%{g}  &   &   &   &   &\x &   &\x &   \\
{h}  &   &    &   &\x &\x     \\
%{i}  &   &\x &   &   &   &   &\x &\x \\
%     %& 1 & 2 & 3 
%     & 4 & 5 & 6 & 7 & 8 \\\hline
%{a}~~%&   &\x &\x 
%     &\x &\x &   &\x &\x \\
%{b}  %&\x &\x &\x 
%     &\x &\x &   &\x &   \\
%{c}  %&   &\x &\x 
%     &   &   &\x &\x &   \\
%%{d}  &   &\x &   &   &   &   &\x &\x \\
%{e}  %&\x &   &\x 
%     &   &\x &\x &\x &   \\
%{f}  %&\x &   &\x    
%     & &\x &\x &\x &   \\
%%{g}  &   &   &   &   &\x &   &\x &   \\
%{h}  %&\x &   &\x 
%     &   &\x &\x &\x &   \\
%%{i}  &   &\x &   &   &   &   &\x &\x \\
\end{tabular}
};


%\begin{tabular}{l|cccccccc}
%     & 1 & 2 & 3 & 4 & 5 & 6 & 7 & \\\hline
%{a}~~&   &\x &\x &\x &\x &   &\x &   \\
%{b}  &\x &\x &\x &\x &\x &   &\x &   \\
%{c}  &   &\x &\x &   &   &\x &\x &   \\
%%{d}  &   &\x &   &   &   &   &\x &\x \\
%{e}  &\x &   &\x &   &\x &\x &\x &   \\
%{f}  &\x &   &\x &   &\x &\x &\x &   \\
%%{g}  &   &   &   &   &\x &   &\x &   \\
%{h}  &   &   &\x &   &\x &\x &\x &   \\
%%{i}  &   &\x &   &   &   &   &\x &\x \\
%%     %& 1 & 2 & 3 
%%     & 4 & 5 & 6 & 7 & 8 \\\hline
%%{a}~~%&   &\x &\x 
%%     &\x &\x &   &\x &\x \\
%%{b}  %&\x &\x &\x 
%%     &\x &\x &   &\x &   \\
%%{c}  %&   &\x &\x 
%%     &   &   &\x &\x &   \\
%%%{d}  &   &\x &   &   &   &   &\x &\x \\
%%{e}  %&\x &   &\x 
%%     &   &\x &\x &\x &   \\
%%{f}  %&\x &   &\x    
%%     & &\x &\x &\x &   \\
%%%{g}  &   &   &   &   &\x &   &\x &   \\
%%{h}  %&\x &   &\x 
%%     &   &\x &\x &\x &   \\
%%%{i}  &   &\x &   &   &   &   &\x &\x \\
%\end{tabular}
%};


\node (d) at (0,-14.5) {%
\begin{tabular}{l|cccc}
     & 4 & 5 & 6  \\\hline
{a}~~&\x &\x &       \\
{b}  &\x &\x &       \\
{c}  &   &   &\x     \\
%{d}  &   &\x &   &   &   &   &\x &\x \\
{e}  &   &\x &\x      \\
{f}  &   &\x &\x    \\
%{g}  &   &   &   &   &\x &   &\x &   \\
{h}  &   &\x &\x     \\
%{i}  &   &\x &   &   &   &   &\x &\x \\
%     %& 1 & 2 & 3 
%     & 4 & 5 & 6 & 7 & 8 \\\hline
%{a}~~%&   &\x &\x 
%     &\x &\x &   &\x &\x \\
%{b}  %&\x &\x &\x 
%     &\x &\x &   &\x &   \\
%{c}  %&   &\x &\x 
%     &   &   &\x &\x &   \\
%%{d}  &   &\x &   &   &   &   &\x &\x \\
%{e}  %&\x &   &\x 
%     &   &\x &\x &\x &   \\
%{f}  %&\x &   &\x    
%     & &\x &\x &\x &   \\
%%{g}  &   &   &   &   &\x &   &\x &   \\
%{h}  %&\x &   &\x 
%     &   &\x &\x &\x &   \\
%%{i}  &   &\x &   &   &   &   &\x &\x \\
\end{tabular}
};


\node[inner xsep=1cm] (e) at (0,-18) {%
\begin{tabular}{l|cccc}
     & 4 & 5 & 6    \\\hline
{a,b}~~&\x &\x &      \\
{c}  &   &   &\x     \\
{e,f,h}  &   &\x &\x      \\
\end{tabular}
};



\node[inner xsep=1cm] (e2) at (10,-18) {%
\begin{tabular}{l|cc|cccc}
    & 1 & 2& 4 & 5 & 6    \\\hline
{a,b}~~& & \x &\x &\x &      \\
{c}  & & \x&   &   &\x     \\
{e,f,h}& &  &   &\x &\x      \\
\end{tabular}
};




%\node (d) at (0,-14) {%
%\begin{tabular}{l|ccccc}
%     %& 1 & 2 & 3 
%     & 4 & 5 & 6 & 8 \\\hline
%{a}~~%&   &\x &\x 
%     &\x &\x &    &\x \\
%{b}  %&\x &\x &\x 
%     &\x &\x &    &   \\
%{c}  %&   &\x &\x 
%     &   &   &\x  &   \\
%%{d}  &   &\x &   &   &   &   &\x &\x \\
%{e}  %&\x &   &\x 
%     &   &\x &\x  &   \\
%{f}  %&\x &   &\x    
%     & &\x &\x  &   \\
%%%{g}  &   &   &   &   &\x &   &\x &   \\
%{h}  %&\x &   &\x 
%     &   &\x &\x  &   \\
%%%{i}  &   &\x &   &   &   &   &\x &\x \\
%\end{tabular}
%};


%\node (e1) at (0,-18) {%
%\begin{tabular}{l|cccc|l}
%     %& 1 & 2 & 3 
%     & 4 & 5 & 6 & 8 \\\hline
%{a}~~%&   &\x &\x 
%     &\x &\x &    &\x &{a} \\
%{b}  %&\x &\x &\x 
%     &\x &\x &    &   &{b}\\
%{c}  %&   &\x &\x 
%     &   &   &\x  &   &{c}\\
%%{d}  &   &\x &   &   &   &   &\x &\x \\
%{e}  %&\x &   &\x 
%     &   &\x &\x  &   &{e,f,g}\\
%%{f}  %&\x &   &\x    
%%     & &\x &\x  &   \\
%%%{g}  &   &   &   &   &\x &   &\x &   \\
%%{h}  %&\x &   &\x 
%%     &   &\x &\x  &   \\
%%%{i}  &   &\x &   &   &   &   &\x &\x \\
%\end{tabular}
%};


%\node (e2) at (5,-20) {%
%\begin{tabular}{l|ccccc}
%     %& 1 & 2 & 3 
%     & 4 & 5 & 6 & 8 \\\hline
%{a}~~%&   &\x &\x 
%     &\x &\x &    &\x \\
%{b}  %&\x &\x &\x 
%     &\x &\x &    &   \\
%{c}  %&   &\x &\x 
%     &   &   &\x  &   \\
%%{d}  &   &\x &   &   &   &   &\x &\x \\
%{e,f,h}  %&\x &   &\x 
%     &   &\x &\x  &   \\
%%{f}  %&\x &   &\x    
%%     & &\x &\x  &   \\
%%%{g}  &   &   &   &   &\x &   &\x &   \\
%%{h}  %&\x &   &\x 
%%     &   &\x &\x  &   \\
%%%{i}  &   &\x &   &   &   &   &\x &\x \\
%\end{tabular}
%};




\draw[-latex] (a) -- node[right,near start,text width=7cm]{
%Restrict to $B^\down$:
\begin{itemize}\item[(a)] Remove objects not in $\{3,7\}^\down$:\\ Objects d,g, and i are removed.
%\item[$\bullet$]
%Remove attributes not in $N$ \eqref{eq:N}. \\
%Attribute $8$ is removed because no object in $\{3,7\}^\down$ has them.\\
%Attributes $3,7$ are removed because they are in $B$
%Attributes $1,2$ are removed as they are lesser than $i=3$.
\end{itemize}
} (b);

\draw[-latex] (b) -- node[right,near start,text width=10cm]{\begin{itemize}\item[(b)] Remove empty and full attributes:\\ Attributes 3, 7, and 8 are removed.\end{itemize}} (c);

\draw[-latex] (c) -- node[right,near start,text width=7cm]{\begin{itemize}\item[(c)] Remove attributes lesser than 3:\\ Attributes 1 and 2 are removed.\end{itemize}} (d);

%
\draw[-latex] (d) -- node[right,near start,text width=5.5cm]{\begin{itemize}\item[(d)] Merge identical objects together.\end{itemize}
} (e);

\draw[-latex] (e) -- node[below,text width=5.5cm]{\begin{itemize}\item[(e)] Add interior intersections.\end{itemize}
} (e2);


%\draw[-latex] (d) -- node[right,near start,text width=5.5cm]{\begin{itemize}\item[4.] Remove duplicate objects.\\ Objects f and h are removed.\end{itemize}
%} (e2);


\end{tikzpicture}
}
\end{center}
\caption{Obtaining contitional context ${\cal K}_{B,y}$ for attribute set $B = \{3,7\}$ and attribute $y=3$.\label{fig:conditionalDB}}
\end{figure}

